Exp-Graph: How Connections Learn Facial Attributes in Graph-based Expression Recognition

Facial expression recognition is crucial for human-computer interaction applications such as face animation, video surveillance, affective computing, medical analysis, etc. Since the structure of facial attributes varies with facial expressions, incorporating structural information into facial attributes is essential for facial expression recognition. In this paper, we propose Exp-Graph, a novel framework designed to represent the structural relationships among facial attributes using graph-based modeling for facial expression recognition. For facial attributes graph representation, facial landmarks are used as the graph's vertices. At the same time, the edges are determined based on the proximity of the facial landmark and the similarity of the local appearance of the facial attributes encoded using the vision transformer. Additionally, graph convolutional networks are utilized to capture and integrate these structural dependencies into the encoding of facial attributes, thereby enhancing the accuracy of expression recognition. Thus, Exp-Graph learns from the facial attribute graphs highly expressive semantic representations. On the other hand, the vision transformer and graph convolutional blocks help the framework exploit the local and global dependencies among the facial attributes that are essential for the recognition of facial expressions. We conducted comprehensive evaluations of the proposed Exp-Graph model on three benchmark datasets: Oulu-CASIA, eNTERFACE05, and AFEW. The model achieved recognition accuracies of 98.09\%, 79.01\%, and 56.39\%, respectively. These results indicate that Exp-Graph maintains strong generalization capabilities across both controlled laboratory settings and real-world, unconstrained environments, underscoring its effectiveness for practical facial expression recognition applications.

==> mathdef.tex <==
\newtheorem{defi}{Definition}
\newtheorem{prop}[defi]{Proposition}
\newtheorem{lemm}[defi]{Lemma}
\newtheorem{theo}[defi]{Theorem}
\newtheorem{coro}[defi]{Corollary}
\newtheorem{exam}[defi]{Example}
%\newtheorem{fact}[defi]{Fact}
\newtheorem{algo}[defi]{Algorithm}
%\newtheorem{claim}[defi]{Claim}
% \newcommand{\theoproof}[1]{\noindent{\bf (Proof of Theorem #1) }}
% \newcommand{\propproof}[1]{\noindent{\bf (Proof of Proposition #1) }}
% \newcommand{\lemmproof}[1]{\noindent{\bf (Proof of Lemma #1) }\\}
% \newcommand{\lemmproofn}[1]{\noindent{\bf (Proof of Lemma #1) }}
% \newcommand{\coroproof}[1]{\noindent{\bf (Proof of Corollary #1) }\\}
%\newcommand{\proof}{\noindent\textbf{(Proof)} }
%\newcommand{\proofend}{\hfill$\Box$\vspace{2mm}}
% \newcommand{\QED}{\rule{7pt}{7pt}}

\newcommand{\sgn}{\mathrm{sgn}}
\newcommand{\define}{\stackrel{\mathrm{def}}{=}}
\newcommand{\argmin}{\mathop{\mathrm{argmin\,}}}
\newcommand{\argmax}{\mathop{\mathrm{argmax\,}}}
\newcommand{\rank}[1]{\mathrm{rank}\left(#1\right)}
\newcommand{\tr}[1]{\mathrm{tr}(#1)}
\newcommand{\diag}[1]{\mathrm{diag}\left(#1\right)}
\newcommand{\sinc}{\mathrm{sinc}\;}
\newcommand{\unorm}[1]{\|#1\|}
\newcommand{\unorms}[1]{\unorm{#1}^2}
\newcommand{\inner}[2]{\langle #1,#2\rangle}
\newcommand{\iid}{\stackrel{\mathrm{i.i.d.}}{\sim}}
\newcommand{\indep}{\mathop{\perp\!\!\!\perp}}

\newcommand{\pnu}{p}
\newcommand{\pde}{p'}
\newcommand{\Pnu}{P}
\newcommand{\Pde}{P'}
\newcommand{\pmix}{q_\alpha}
\newcommand{\numparams}{n}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55

\newcommand{\mathbbC}{\mathbb{C}}
\newcommand{\mathbbE}{\mathbb{E}}
\newcommand{\mathbbN}{\mathbb{N}}
\newcommand{\mathbbR}{\mathbb{R}}
\newcommand{\mathbbS}{\mathbb{S}}

\newcommand{\boldzero}{{\boldsymbol{0}}}
\newcommand{\boldone}{{\boldsymbol{1}}}

\newcommand{\boldA}{{\boldsymbol{A}}}
\newcommand{\boldB}{{\boldsymbol{B}}}
\newcommand{\boldC}{{\boldsymbol{C}}}
\newcommand{\boldD}{{\boldsymbol{D}}}
\newcommand{\boldE}{{\boldsymbol{E}}}
\newcommand{\boldF}{{\boldsymbol{F}}}
\newcommand{\boldG}{{\boldsymbol{G}}}
\newcommand{\boldH}{{\boldsymbol{H}}}
\newcommand{\boldI}{{\boldsymbol{I}}}
\newcommand{\boldJ}{{\boldsymbol{J}}}
\newcommand{\boldK}{{\boldsymbol{K}}}
\newcommand{\boldL}{{\boldsymbol{L}}}
\newcommand{\boldM}{{\boldsymbol{M}}}
\newcommand{\boldN}{{\boldsymbol{N}}}
\newcommand{\boldO}{{\boldsymbol{O}}}
\newcommand{\boldP}{{\boldsymbol{P}}}
\newcommand{\boldQ}{{\boldsymbol{Q}}}
\newcommand{\boldR}{{\boldsymbol{R}}}
\newcommand{\boldS}{{\boldsymbol{S}}}
\newcommand{\boldT}{{\boldsymbol{T}}}
\newcommand{\boldU}{{\boldsymbol{U}}}
\newcommand{\boldV}{{\boldsymbol{V}}}
\newcommand{\boldW}{{\boldsymbol{W}}}
\newcommand{\boldX}{{\boldsymbol{X}}}
\newcommand{\boldY}{{\boldsymbol{Y}}}
\newcommand{\boldZ}{{\boldsymbol{Z}}}

\newcommand{\bolda}{{\boldsymbol{a}}}
\newcommand{\boldb}{{\boldsymbol{b}}}
\newcommand{\boldc}{{\boldsymbol{c}}}
\newcommand{\boldd}{{\boldsymbol{d}}}
\newcommand{\bolde}{{\boldsymbol{e}}}
\newcommand{\boldf}{{\boldsymbol{f}}}
\newcommand{\boldg}{{\boldsymbol{g}}}
\newcommand{\boldh}{{\boldsymbol{h}}}
\newcommand{\boldi}{{\boldsymbol{i}}}
\newcommand{\boldj}{{\boldsymbol{j}}}
\newcommand{\boldk}{{\boldsymbol{k}}}
\newcommand{\boldl}{{\boldsymbol{l}}}
\newcommand{\boldm}{{\boldsymbol{m}}}
\newcommand{\boldn}{{\boldsymbol{n}}}
\newcommand{\boldo}{{\boldsymbol{o}}}
\newcommand{\boldp}{{\boldsymbol{p}}}
\newcommand{\boldq}{{\boldsymbol{q}}}
\newcommand{\boldr}{{\boldsymbol{r}}}
\newcommand{\bolds}{{\boldsymbol{s}}}
\newcommand{\boldt}{{\boldsymbol{t}}}
\newcommand{\boldu}{{\boldsymbol{u}}}
\newcommand{\boldv}{{\boldsymbol{v}}}
\newcommand{\boldw}{{\boldsymbol{w}}}
\newcommand{\boldx}{{\boldsymbol{x}}}
\newcommand{\boldy}{{\boldsymbol{y}}}
\newcommand{\boldz}{{\boldsymbol{z}}}

\newcommand{\boldztr}{\boldz^{\mathrm{tr}}}
\newcommand{\boldzte}{\boldz^{\mathrm{te}}}


\newcommand{\boldalpha}{{\boldsymbol{\alpha}}}
\newcommand{\boldbeta}{{\boldsymbol{\beta}}}
\newcommand{\boldgamma}{{\boldsymbol{\gamma}}}
\newcommand{\bolddelta}{{\boldsymbol{\delta}}}
\newcommand{\boldepsilon}{{\boldsymbol{\epsilon}}}
\newcommand{\boldzeta}{{\boldsymbol{\zeta}}}
\newcommand{\boldeta}{{\boldsymbol{\eta}}}
\newcommand{\boldtheta}{{\boldsymbol{\theta}}}
\newcommand{\boldiota}{{\boldsymbol{\iota}}}
\newcommand{\boldkappa}{{\boldsymbol{\kappa}}}
\newcommand{\boldlambda}{{\boldsymbol{\lambda}}}
\newcommand{\boldmu}{{\boldsymbol{\mu}}}
\newcommand{\boldnu}{{\boldsymbol{\nu}}}
\newcommand{\boldxi}{{\boldsymbol{\xi}}}
\newcommand{\boldpi}{{\boldsymbol{\pi}}}
\newcommand{\boldrho}{{\boldsymbol{\rho}}}
\newcommand{\boldsigma}{{\boldsymbol{\sigma}}}
\newcommand{\boldtau}{{\boldsymbol{\tau}}}
\newcommand{\boldupsilon}{{\boldsymbol{\upsilon}}}
\newcommand{\boldphi}{{\boldsymbol{\phi}}}
\newcommand{\boldchi}{{\boldsymbol{\chi}}}
\newcommand{\boldpsi}{{\boldsymbol{\psi}}}
\newcommand{\boldomega}{{\boldsymbol{\omega}}}
\newcommand{\boldGamma}{{\boldsymbol{\Gamma}}}
\newcommand{\boldDelta}{{\boldsymbol{\Delta}}}
\newcommand{\boldTheta}{{\boldsymbol{\Theta}}}
\newcommand{\boldLambda}{{\boldsymbol{\Lambda}}}
\newcommand{\boldXi}{{\boldsymbol{\Xi}}}
\newcommand{\boldPi}{{\boldsymbol{\Pi}}}
\newcommand{\boldSigma}{{\boldsymbol{\Sigma}}}
\newcommand{\boldUpsilon}{{\boldsymbol{\Upsilon}}}
\newcommand{\boldPhi}{{\boldsymbol{\Phi}}}
\newcommand{\boldPsi}{{\boldsymbol{\Psi}}}
\newcommand{\boldOmega}{{\boldsymbol{\Omega}}}
\newcommand{\boldvarepsilon}{{\boldsymbol{\varepsilon}}}
\newcommand{\boldvartheta}{{\boldsymbol{\vartheta}}}
\newcommand{\boldvarpi}{{\boldsymbol{\varpi}}}
\newcommand{\boldvarrho}{{\boldsymbol{\varrho}}}
\newcommand{\boldvarsigma}{{\boldsymbol{\varsigma}}}
\newcommand{\boldvarphi}{{\boldsymbol{\varphi}}}
 
\newcommand{\calA}{{\mathcal{A}}}
\newcommand{\calB}{{\mathcal{B}}}
\newcommand{\calC}{{\mathcal{C}}}
\newcommand{\calD}{{\mathcal{D}}}
\newcommand{\calE}{{\mathcal{E}}}
\newcommand{\calF}{{\mathcal{F}}}
\newcommand{\calG}{{\mathcal{G}}}
\newcommand{\calH}{{\mathcal{H}}}
\newcommand{\calI}{{\mathcal{I}}}
\newcommand{\calJ}{{\mathcal{J}}}
\newcommand{\calK}{{\mathcal{K}}}
\newcommand{\calL}{{\mathcal{L}}}
\newcommand{\calM}{{\mathcal{M}}}
\newcommand{\calN}{{\mathcal{N}}}
\newcommand{\calO}{{\mathcal{O}}}
\newcommand{\calP}{{\mathcal{P}}}
\newcommand{\calQ}{{\mathcal{Q}}}
\newcommand{\calR}{{\mathcal{R}}}
\newcommand{\calS}{{\mathcal{S}}}
\newcommand{\calT}{{\mathcal{T}}}
\newcommand{\calU}{{\mathcal{U}}}
\newcommand{\calV}{{\mathcal{V}}}
\newcommand{\calW}{{\mathcal{W}}}
\newcommand{\calX}{{\mathcal{X}}}
\newcommand{\calY}{{\mathcal{Y}}}
\newcommand{\calZ}{{\mathcal{Z}}}

\newcommand{\calXtr}{{\mathcal{X}^{\mathrm{tr}}}}
\newcommand{\calYtr}{{\mathcal{Y}^{\mathrm{tr}}}}
\newcommand{\calXte}{{\mathcal{X}^{\mathrm{te}}}}
\newcommand{\calYte}{{\mathcal{Y}^{\mathrm{te}}}}

\newcommand{\thetah}{{\widehat{\theta}}}
\newcommand{\thetat}{{\widetilde{\theta}}}
\newcommand{\boldthetah}{{\widehat{\boldtheta}}}
\newcommand{\boldthetat}{{\widetilde{\boldtheta}}}
\newcommand{\boldzetah}{{\widehat{\boldzeta}}}
\newcommand{\calAh}{{\widehat{\calA}}}
\newcommand{\boldEh}{{\widehat{\boldE}}}
\newcommand{\boldGh}{{\widehat{\boldG}}}
\newcommand{\boldUh}{{\widehat{\boldU}}}
\newcommand{\Eh}{{\widehat{E}}}
\newcommand{\jh}{{\widehat{j}}}
\newcommand{\boldbetah}{{\widehat{\boldbeta}}}
\newcommand{\boldbetat}{{\widetilde{\boldbeta}}}

\newcommand{\mathrmd}{{\mathrm{d}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\domainx}{\calX}
\newcommand{\domainy}{\calY}
\newcommand{\domainz}{\calZ}
\newcommand{\inputdim}{d}
\newcommand{\reducedim}{m}
\newcommand{\reducedimh}{\widehat{\reducedim}}
\newcommand{\ntask}{m}
\newcommand{\nmix}{c}
\newcommand{\inputdimx}{\inputdim_{\mathrm{x}}}
\newcommand{\inputdimy}{\inputdim_{\mathrm{y}}}
\newcommand{\inputdimz}{\inputdim_{\mathrm{z}}}

\newcommand{\ratiosymbol}{r}
\newcommand{\ratio}{\ratiosymbol}
\newcommand{\ratioh}{\widehat{\ratiosymbol}}
\newcommand{\ratiomodel}{\ratiosymbol_{\alpha}}
\newcommand{\relratio}{\ratio_{\alpha}}

\newcommand{\densitysymbol}{p}
\newcommand{\cumulativesymbol}{P}
\newcommand{\density}{\densitysymbol^\ast}
\newcommand{\densitynu}{\densitysymbol_{\mathrm{te}}^\ast}
\newcommand{\densityde}{\densitysymbol_{\mathrm{de}}^\ast}
\newcommand{\densitydet}{\widetilde{\densitysymbol}_{\mathrm{de}}^\ast}
\newcommand{\cumulativede}{\cumulativesymbol_{\mathrm{de}}^\ast}
\newcommand{\cumulativenu}{\cumulativesymbol_{\mathrm{te}}^\ast}
\newcommand{\cumulativedeh}{\widehat{\cumulativesymbol}_{\mathrm{de}}}
\newcommand{\densityh}{\widehat{\densitysymbol}}
\newcommand{\densityt}{\widetilde{\densitysymbol}}
\newcommand{\densitynuh}{\widehat{\densitysymbol}_{\mathrm{te}}}
\newcommand{\densitydeh}{\widehat{\densitysymbol}_{\mathrm{de}}}
%\newcommand{\densitymodelnu}{\densitysymbol_{\mathrm{te}}}
%\newcommand{\densitymodelde}{\densitysymbol_{\mathrm{de}}}
\newcommand{\densitymodel}{\densitysymbol}
\newcommand{\prior}{\pi}
\newcommand{\posterior}{\densitysymbol}
\newcommand{\evidence}{\densitysymbol}

\newcommand{\xy}{\mathrm{xy}}
\newcommand{\zy}{\mathrm{zy}}
\newcommand{\x}{\boldsymbol{x}}
\newcommand{\y}{\boldsymbol{y}}


\newcommand{\ptr}{p_{\mathrm{tr}}}
\newcommand{\pte}{p_{\mathrm{te}}}
\newcommand{\pxy}{p_{\mathrm{x,y}}}
\newcommand{\pzy}{p_{\mathrm{z,y}}}
\newcommand{\px}{p_{\mathrm{x}}}
\newcommand{\pz}{p_{\mathrm{z}}}
\newcommand{\py}{p_{\mathrm{y}}}
\newcommand{\boldxtr}{\boldx^{\mathrm{tr}}}
\newcommand{\boldxte}{\boldx^{\mathrm{te}}}
\newcommand{\xtr}{x^{\mathrm{tr}}}
\newcommand{\xte}{x^{\mathrm{te}}}
\newcommand{\ytr}{y^{\mathrm{tr}}}
\newcommand{\yte}{y^{\mathrm{te}}}
\newcommand{\epsilontr}{\epsilon^{\mathrm{tr}}}
\newcommand{\epsilonte}{\epsilon^{\mathrm{te}}}
\newcommand{\ntr}{n_{\mathrm{tr}}}
\newcommand{\nte}{n_{\mathrm{te}}}
\newcommand{\nteu}{n_{\mathrm{te}}'}
\newcommand{\ntep}{n_{\mathrm{te}}}
\newcommand{\densitytr}{\densitysymbol_{\mathrm{tr}}^\ast}
\newcommand{\densityte}{\densitysymbol_{\mathrm{te}}^\ast}
\newcommand{\Xtr}{X^{\mathrm{tr}}}
\newcommand{\Xte}{X^{\mathrm{te}}}
\newcommand{\boldXtr}{\boldX^{\mathrm{tr}}}
\newcommand{\boldXte}{\boldX^{\mathrm{te}}}
\newcommand{\boldytr}{\boldy^{\mathrm{tr}}}
\newcommand{\boldyte}{\boldy^{\mathrm{te}}}
\newcommand{\Gen}{G}
\newcommand{\Genh}{\widehat{\Gen}}

\newcommand{\boldxnu}{\boldx^{\mathrm{te}}}
\newcommand{\boldxde}{\boldx^{\mathrm{tr}}}
\newcommand{\boldxt}{\widetilde{\boldx}}

\newcommand{\boldunu}{\boldu^{\mathrm{te}}}
\newcommand{\boldude}{\boldu^{\mathrm{tr}}}
\newcommand{\boldvnu}{\boldv^{\mathrm{te}}}
\newcommand{\boldvde}{\boldv^{\mathrm{tr}}}
\newcommand{\boldunuh}{\widehat{\boldu}^{\mathrm{te}}}
\newcommand{\boldudeh}{\widehat{\boldu}^{\mathrm{tr}}}
\newcommand{\unu}{u^{\mathrm{te}}}
\newcommand{\ude}{u^{\mathrm{tr}}}

\newcommand{\nde}{n_{\mathrm{tr}}}
\newcommand{\nnu}{n_{\mathrm{te}}}
\newcommand{\nsample}{n}

\newcommand{\nparam}{b}
\newcommand{\nparamm}{t}
\newcommand{\nclass}{c}
\newcommand{\ndet}{\widetilde{n}_{\mathrm{tr}}}

\newcommand{\data}{D}
\newcommand{\datanu}{D^{\mathrm{te}}}
\newcommand{\datade}{D^{\mathrm{tr}}}

\newcommand{\boldratiosymbol}{\boldr}
\newcommand{\boldratio}{\boldratiosymbol^\ast}
\newcommand{\boldratiomodel}{{\boldratiosymbol}}
\newcommand{\boldratiode}{\boldratiosymbol_{\mathrm{tr}}^\ast}
\newcommand{\boldrationu}{\boldratiosymbol_{\mathrm{te}}^\ast}
\newcommand{\boldratioh}{\widehat{\boldratiosymbol}}
\newcommand{\boldratiodeh}{\boldratioh_{\mathrm{tr}}}
\newcommand{\boldrationuh}{\boldratioh_{\mathrm{te}}}
\newcommand{\boldratiodemodel}{\boldratiomodel_{\mathrm{tr}}}
\newcommand{\boldrationumodel}{\boldratiomodel_{\mathrm{te}}}
\newcommand{\boldPhide}{\boldPhi_{\mathrm{tr}}}
\newcommand{\boldPhinu}{\boldPhi_{\mathrm{te}}}
\newcommand{\boldPside}{\boldPsi_{\mathrm{tr}}}
\newcommand{\boldPsinu}{\boldPsi_{\mathrm{te}}}

\newcommand{\Bregman}{\mathrm{BR}}
\newcommand{\fdivergence}{\mathrm{ASC}}

% \newcommand{\fh}{\widehat{f}}
%\newcommand{\function}{f^\ast}
\newcommand{\functionmodel}{f}
\newcommand{\functionh}{\widehat{f}}

\newcommand{\xde}{x^{\mathrm{tr}}}
\newcommand{\xdet}{\widetilde{x}^{\mathrm{tr}}}
\newcommand{\xnu}{x^{\mathrm{te}}}
\newcommand{\zde}{z^{\mathrm{tr}}}
\newcommand{\boldxdet}{\widetilde{\boldx}^{\mathrm{tr}}}
\newcommand{\boldxnut}{\widetilde{\boldx}^{\mathrm{te}}}
\newcommand{\etade}{\eta^{\mathrm{tr}}}
\newcommand{\etanu}{\eta^{\mathrm{te}}}
\newcommand{\boldepsilonde}{\boldepsilon^{\mathrm{tr}}}
\newcommand{\boldepsilondet}{\widetilde{\boldepsilon}^{\mathrm{tr}}}
\newcommand{\epsilonde}{\epsilon^{\mathrm{tr}}}
\newcommand{\epsilonnu}{\epsilon^{\mathrm{te}}}
\newcommand{\epsilondeh}{\widehat{\epsilon}^{\mathrm{tr}}}
\newcommand{\epsilondet}{\widetilde{\epsilon}^{\mathrm{tr}}}
\newcommand{\boldrde}{\boldr^{\mathrm{tr}}}
\newcommand{\boldrnu}{\boldr^{\mathrm{te}}}
\newcommand{\Ade}{A^{\mathrm{tr}}}
\newcommand{\Anu}{A^{\mathrm{te}}}
\newcommand{\Xde}{X^{\mathrm{tr}}}
\newcommand{\Xdet}{\widetilde{X}^{\mathrm{tr}}}
\newcommand{\Xnu}{X^{\mathrm{te}}}
\newcommand{\boldXde}{\boldX^{\mathrm{tr}}}
\newcommand{\boldXdet}{\widetilde{\boldX}^{\mathrm{tr}}}
\newcommand{\boldXnu}{\boldX^{\mathrm{te}}}
\newcommand{\boldGde}{\boldG^{\mathrm{tr}}}
\newcommand{\boldGnu}{\boldG^{\mathrm{te}}}
\newcommand{\boldAde}{\boldA^{\mathrm{tr}}}
\newcommand{\boldAnu}{\boldA^{\mathrm{te}}}
\newcommand{\boldKdede}{\boldK_{\mathrm{tr},\mathrm{tr}}}
\newcommand{\boldKdenu}{\boldK_{\mathrm{tr},\mathrm{te}}}
\newcommand{\boldKde}{\boldK_{\mathrm{tr}}}
\newcommand{\boldKnu}{\boldK_{\mathrm{te}}}
\newcommand{\boldyde}{\boldy^{\mathrm{tr}}}
\newcommand{\boldydet}{\widetilde{\boldy}^{\mathrm{tr}}}
\newcommand{\Kdede}{K_{\mathrm{tr},\mathrm{tr}}}
\newcommand{\Kdenu}{K_{\mathrm{tr},\mathrm{te}}}
\newcommand{\Kde}{K_{\mathrm{tr}}}
\newcommand{\yde}{y^{\mathrm{tr}}}
\newcommand{\ydet}{\widetilde{y}^{\mathrm{tr}}}
\newcommand{\ynu}{y^{\mathrm{te}}}
\newcommand{\yh}{\widehat{y}}
\newcommand{\ynuh}{\widehat{y}^{\mathrm{te}}}
\newcommand{\calXde}{\calX^{\mathrm{tr}}}
\newcommand{\calYde}{\calY^{\mathrm{tr}}}
\newcommand{\calZde}{\calZ^{\mathrm{tr}}}
\newcommand{\calXnu}{\calX^{\mathrm{te}}}
\newcommand{\calYnu}{\calY^{\mathrm{te}}}
\newcommand{\calZnu}{\calZ^{\mathrm{te}}}
\newcommand{\calZt}{\widetilde{\calZ}}

\newcommand{\Pb}{{P^{\ast}}'}
\newcommand{\Pa}{P^\ast}
\newcommand{\pb}{{p^{\ast}}'}
\newcommand{\pa}{p^\ast}
\newcommand{\nb}{n'}
\newcommand{\na}{n}
\newcommand{\calXb}{\calX'}
\newcommand{\calXa}{\calX}
\newcommand{\calXbt}{\widetilde{\calX}'}
\newcommand{\calXat}{\widetilde{\calX}}
\newcommand{\boldxb}{\boldx'}
\newcommand{\boldxa}{\boldx}
\newcommand{\boldHhde}{{\widehat{\boldH}}}
\newcommand{\boldhhde}{{\widehat{\boldh}}'}
\newcommand{\boldhhnu}{{\widehat{\boldh}}}
\newcommand{\boldGhde}{{\widehat{\boldG}}}
\newcommand{\boldghde}{{\widehat{\boldg}}'}
\newcommand{\boldghnu}{{\widehat{\boldg}}}
\newcommand{\nn}{\overline{n}}

\newcommand{\boldTh}{{\widehat{\boldT}}}
\newcommand{\boldgh}{{\widehat{\boldg}}}
\newcommand{\boldHh}{{\widehat{\boldH}}}
\newcommand{\boldhh}{{\widehat{\boldh}}}
\newcommand{\boldBh}{{\widehat{\boldB}}}
\newcommand{\Hh}{{\widehat{H}}}
\newcommand{\hh}{{\widehat{h}}}
\newcommand{\boldHt}{{\widetilde{\boldH}}}
\newcommand{\boldht}{{\widetilde{\boldh}}}
\newcommand{\boldDt}{{\widetilde{\boldD}}}
\newcommand{\boldWt}{{\widetilde{\boldW}}}
\newcommand{\boldXt}{{\widetilde{\boldX}}}
\newcommand{\Wt}{{\widetilde{W}}}
\newcommand{\Dt}{{\widetilde{D}}}
\newcommand{\Qt}{{\widetilde{Q}}}
\newcommand{\Qh}{{\widehat{Q}}}
\newcommand{\Ht}{{\widetilde{H}}}
\newcommand{\Xt}{{\widetilde{X}}}
\newcommand{\Jh}{\widehat{J}}
\newcommand{\Jt}{\widetilde{J}}
\newcommand{\Vh}{\widehat{V}}
\newcommand{\Fh}{\widehat{F}}
\newcommand{\Gh}{\widehat{G}}
\newcommand{\KL}{\mathrm{KL}}
\newcommand{\KLh}{\widehat{\KL}}
\newcommand{\KLt}{\widetilde{\KL}}
\newcommand{\boldxih}{\widehat{\boldxi}}
\newcommand{\boldalphah}{\widehat{\boldalpha}}
\newcommand{\boldalphat}{\widetilde{\boldalpha}}
\newcommand{\alphah}{\widehat{\alpha}}
\newcommand{\sigmah}{{\widehat{\sigma}}}
\newcommand{\lambdah}{{\widehat{\lambda}}}

\newcommand{\boldSb}{\boldS^{\mathrm{b}}}
\newcommand{\boldSw}{\boldS^{\mathrm{w}}}
\newcommand{\boldWb}{\boldW^{\mathrm{b}}}
\newcommand{\boldWw}{\boldW^{\mathrm{w}}}
\newcommand{\Wb}{W^{\mathrm{b}}}
\newcommand{\Ww}{W^{\mathrm{w}}}
\newcommand{\boldSlb}{\boldS^{\mathrm{lb}}}
\newcommand{\boldSlw}{\boldS^{\mathrm{lw}}}
\newcommand{\boldWlb}{\boldW^{\mathrm{lb}}}
\newcommand{\boldWlw}{\boldW^{\mathrm{lw}}}
\newcommand{\Wlb}{W^{\mathrm{lb}}}
\newcommand{\Wlw}{W^{\mathrm{lw}}}
\newcommand{\weight}{w}
\newcommand{\weighth}{\widehat{w}}


%\newcommand{\resample}{\omega}
\newcommand{\resample}{\zeta}
\newcommand{\CEVOW}{\textrm{CV}_\textrm{W}}
\newcommand{\PCEVOW}{\textrm{PCV}_\textrm{W}}
\newcommand{\CEVOO}{\textrm{CV}_\textrm{O}}
\newcommand{\PCEVOO}{\textrm{PCV}_\textrm{O}}
\newcommand{\FEVOW}{\textrm{FV}_\textrm{W}}
\newcommand{\PFEVOW}{\textrm{PFV}_\textrm{W}}
\newcommand{\FEBVOW}{\textrm{FBV}_\textrm{OW}}
\newcommand{\PFEBVOW}{\textrm{PFBV}_\textrm{OW}}
\newcommand{\ALICE}{\textrm{ALICE}}
\newcommand{\PALICE}{\textrm{PALICE}}

\newcommand{\model}{M}
\newcommand{\GhatAL}{\Genh^{(AL)}}
\newcommand{\GhatMS}{\Genh^{(MS)}}
\newcommand{\GhatuCEAL}{\Genh^{(EAL)}}
\newcommand{\GhatCEAL}{\Genh^{(nEAL)}}

\newcommand{\hatgn}{\widehat{g}_n}
\newcommand{\gnstar}{g_n^*}
\newcommand{\alzn}{\alpha_0^n}
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\gzn}{\ratio}
\newcommand{\Gconv}{\mathcal{G}^{(\mathrm{c})}}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End:
